Predicting Privacy Preferences for Smart Devices as Norms

Smart devices, such as smart speakers, are becoming ubiquitous, and users expect these devices to act in accordance with their preferences. In particular, since these devices gather and manage personal data, users expect them to adhere to their privacy preferences. However, the current approach of gathering these preferences consists in asking the users directly, which usually triggers automatic responses failing to capture their true preferences. In response, in this paper we present a collaborative filtering approach to predict user preferences as norms. These preference predictions can be readily adopted or can serve to assist users in determining their own preferences. Using a dataset of privacy preferences of smart assistant users, we test the accuracy of our predictions.

==> 02.Motivation.tex <==
\section{Motivation: Smart Personal Assistants}
\label{sec:mot}

%As explained in the introduction, privacy preferences are the paradigmatic example of the problem we try to address in this paper. 
A particular platform in which capturing privacy preferences is challenging and yet essential is that of smart speakers and other smart personal assistants. These devices have benefited from widespread early adoption, and it is estimated that 500 million units were installed in the last quarter of 2021~\cite{Strategy2021smartspeakerinstalled}. Nonetheless, the early adoption of these technologies means that they still have several vulnerabilities that pose a threat to the security and privacy of their users \cite{EduSPASurvey}. Indeed, there have already been cases reported in which smart assistants have not functioned as expected; for example, \cite{GuardianAlexa} reports a case in which a smart speaker recorded and sent a private conversation without the user's consent. These situations hinder user trust in the technology and can ultimately lead users to limit the functionalities of the devices they use, or even to adopting coping mechanisms \cite{Abdi2019More}.

%Hereafter, we present a running example to illustrate each of the concepts we introduce along the paper. 

%\begin{myexample}
%\label{ex:first}
%Consider three users $u_1$, $u_2$, and $u_3$, who have AI assistants. To be concise, these users can define three different preferences, with regard to sharing data with the AI assistant manufacturer, sharing data with their internet provider, and sharing data with developers of third party skills. When it comes to preferences, users $u_1$ and $u_2$, while $u_3$ does not mind sharing data with manufacturers and developers but does not want to share it with the internet provider. Their assistants though, only have partial knowledge of these preferences, $u_1$'s assistant does not know the preference on sharing data with third party skills, $u_2$'s assistant does not know the preference on sharing data with the internet provider, and the same applies to $u_3$'s assistant. Our aim here is for the AI assistants of the users to infer preferences from each other and have complete knowledge of the user's preferences without needing user interaction.
%\end{myexample}
